Hear "No Evil", See "Kenansville": Efficient and Transferable Black-Box Attacks on Speech Recognition and Voice Identification Systems

Automatic speech recognition and voice identification systems are being deployed in a wide array of applications, from providing control mechanisms to devices lacking traditional interfaces, to the automatic transcription of conversations and authentication of users. Many of these applications have significant security and privacy considerations. We develop attacks that force mistranscription and misidentification in state of the art systems, with minimal impact on human comprehension. Processing pipelines for modern systems are comprised of signal preprocessing and feature extraction steps, whose output is fed to a machine-learned model. Prior work has focused on the models, using white-box knowledge to tailor model-specific attacks. We focus on the pipeline stages before the models, which (unlike the models) are quite similar across systems. As such, our attacks are black-box and transferable, and demonstrably achieve mistranscription and misidentification rates as high as 100% by modifying only a few frames of audio. We perform a study via Amazon Mechanical Turk demonstrating that there is no statistically significant difference between human perception of regular and perturbed audio. Our findings suggest that models may learn aspects of speech that are generally not perceived by human subjects, but that are crucial for model accuracy. We also find that certain English language phonemes (in particular, vowels) are significantly more susceptible to our attack. We show that the attacks are effective when mounted over cellular networks, where signals are subject to degradation due to transcoding, jitter, and packet loss.

==> figures/Speech_MSE_Graphs.tex <==
% !TEX root = ../transcription_evasion.tex
\begin{figure}  
  \centering
  \includegraphics[width=1\columnwidth]{figures/word_atk_MSE.png}
  % \caption{The figure shows the effectiveness of the attack methods against
  % different models. The red vertical line shows the audio perceptibility
  % threshold. Audio on the left side of the black vertical line is easily
  % understood by a human listener. The test set comprises of 1000 words. The
  % optimum attack audio is generated for each word. The optimum attack audio
  % has the least distortion, calculated using the MSE and is also
  % mis-transcribed by the model. Black line 50\% attack success}
  \caption{Success of our word-level attack plotted against increasing
  distortion, calculated using Mean Square Error (MSE). The SSA-based
  word-level attack sees a faster, sharper increase in attack success than the
  DFT-based word-level attack, noted by its ability to reach 50\% attack
  success (solid black line) across all models within a smaller span of
  distortion. In every case, the test set accuracy falls considerably before
  reaching the GSM baseline distortion (dashed red line).}
  \label{fig:word_atk_MSE}
  \vspace{-1em}
\end{figure}


==> figures/atk_audio_vs_og_audio_FFT.tex <==
\begin{figure}
  \includegraphics[width=0.5\textwidth]{figures/atk_audio_vs_og_audio_FFT.pdf}
  \caption{The time and frequency domain representation of the attack audio and the original audio. Though there is an imprecipitable change in the time domain, the quantization step discards some frequencies. this can be observed in the frequency representation of the two audios.}
  \label{fig:atk_audio_vs_og_audio_FFT}
\end{figure}

==> figures/atk_vs_og_trans.tex <==

\begin{figure} 
  \includegraphics[width=0.5\textwidth]{figures/atk_vs_og_trans.png}
  \caption{The Google Client transcription of the original and the attack audio. The SSA attack is used to perturb a single phoneme circled in the sentence. All the words following the perturbed phoneme were mistranscribed as well. single phoneme perturbation caused the model to mis-transcribe all the words. The red shows the text that was either lost or added to the original transcription.}
  \label{fig:atk_vs_og_trans}
\end{figure}


==> figures/perturb_fft_sphinx.tex <==
\begin{figure} 
  \includegraphics[width=0.5\textwidth]{figures/perturb_fft_sphinx_fig.png}
  \caption{For each of the 1000 optimum attack audio files we find the spectral difference with its corresponding original audio. We then sum the spectral differences. This shows the areas that were perturbed. The y-axis is scaled between 0 and 1. The distortion is happening across the entire frequency band. This implies that the model's feature extraction weights are do not correctly correspond to the human ear.}
  \label{fig:perturb_fft_sphinx}
\end{figure}


==> figures/phoneme_comp_ee.tex <==

% \begin{figure} 
% \centering
%   \vspace{-1em}

%   \includegraphics[width=0.5\textwidth,height=0.5\textheight]{figures/phoneme_comp.png}
%   \vspace{-1em}

%   \caption{Phoneme vulnerability for a selected model (Wit) using our SSA-based phoneme-level attack. All phonemes are vulnerable to this attack.}
%   \label{fig:phoneme_comp}
%   \vspace{-1em}
% \end{figure}


\begin{figure} 
	\centering

    \subfloat[t][FFT Attack Results.]{\includegraphics[width=0.8\columnwidth]{figures/phoneme_comp_EE_fft.pdf}}
	\qquad
    % \hspace{0.2cm}
    \subfloat[t][SSA Attack Results]{\includegraphics[width=0.8\columnwidth]{figures/phoneme_comp_EE_ssa.pdf}}

  \caption{Phoneme vulnerability for the target models using our phoneme-level attacks. All phonemes are vulnerable to these attacks.}

 \label{fig:phoneme_comp_ee}
  % \vspace{-1em}

\end{figure}

==> figures/phoneme_comp_fft.tex <==

\begin{figure} 
\centering
  \vspace{-1em}
  \includegraphics[width=0.5\textwidth]{figures/phoneme_comp_fig.png}
  \vspace{-1em}

  \caption{Comparison of phoneme threshold between four selected models using our DFT-based phoneme-level attack. There is no discernible relationship between the threshold and the phoneme.}
  \label{fig:phoneme_comp_fft}
  \vspace{-1em}
\end{figure}


==> figures/phoneme_comp_ssa.tex <==

\begin{figure} 
\centering
  \vspace{-1em}

  \includegraphics[width=0.5\textwidth,height=0.3\textheight]{figures/phoneme_comp_fig.png}
  \vspace{-1em}

  \caption{Phoneme vulnerability for a selected model (Wit) using our SSA-based phoneme-level attack. All phonemes are vulnerable to this attack.}
  \label{fig:phoneme_comp_ssa}
  \vspace{-1em}
\end{figure}


==> figures/word_atk_MSE_old.tex <==
% !TEX root = ../transcription_evasion.tex
\begin{figure}  
  \centering
  \includegraphics[width=1\columnwidth]{figures/word_atk_MSE.png}
  % \caption{The figure shows the effectiveness of the attack methods against
  % different models. The red vertical line shows the audio perceptibility
  % threshold. Audio on the left side of the black vertical line is easily
  % understood by a human listener. The test set comprises of 1000 words. The
  % optimum attack audio is generated for each word. The optimum attack audio
  % has the least distortion, calculated using the MSE and is also
  % mis-transcribed by the model. Black line 50\% attack success}
  \caption{Success of our word-level attack plotted against increasing
  distortion, calculated using Mean Square Error (MSE). The SSA-based
  word-level attack sees a faster, sharper increase in attack success than the
  DFT-based word-level attack, noted by its ability to reach 50\% attack
  success (solid black line) across all models within a smaller span of
  distortion. In every case, the test set accuracy falls considerably before
  reaching the GSM baseline distortion (dashed red line).}
  \label{fig:word_atk_MSE}
  \vspace{-1em}
\end{figure}

